QCD parameters and SM-high precisions from $e^+e^-\to$ Hadrons : Summary

In this talk, I summarize the results obtained recently in Ref.\,\cite{SNe} using the PDG 22 compilation of the $e^+e^-\to$ Hadrons $\oplus$ the recent CMD3 data for the pion form factor. Using the gluon condensate $\langle \alpha_s G^2\rangle=(6.49\pm 0.35)\times 10^{-2}$ GeV$^4$ from heavy quark sum rules, the extracted QCD four-quark and dimension eight condensate condensates values are: $\rho\alpha_s\langle\bar\psi\psi\rangle^2= (5.98\pm 0.64)\times 10^{-4}$ GeV$^6$ and $d_8= (4.3\pm 3.0)\times 10^{-2}$ GeV$^8$ from the ratio ${\cal R}_{10}$ of Laplace sum rules to order $\alpha_s^4$. Inversely using these estimated values of the condensates, we obtain from ${\cal R}_{10}$: $\langle \alpha_s G^2\rangle=(6.12\pm 0.61)\times 10^{-2}$ GeV$^4$ which leads to the average $(6.40\pm 0.30)\times 10^{-2}$ GeV$^4$. %from light and heavy quark systems. Using the lowest $\tau$-like decay moment, the mean result of Fixed Order (FO) and Contour Improved (CI) PT series within the standard OPE is : $\alpha_s(M_\tau)=0.3385(50)(136)_{syst}$ [resp. $0.3262(37)(78)_{syst}$] to order $\alpha_s^4$ [resp. $\alpha_s^5$] leading to $\alpha_s(M_Z)$=0.1207(17)(3) [resp. 0.1193(11)(3)], while the sum of the non-perturbative contribution at $M_\tau$ is\,: $\delta^V_{NP}(M_\tau)=(2.3\pm 0.2)\times 10^{-2}$. Using the same data, one also obtains the LO hadronic vacuum polarization to the muon and $\tau$ anomalous magnetic moments: $a_\mu\vert^{hvp}_{l.o}= (7036.5\pm 38.9)\times10^{-11}, \, a_\tau\vert^{hvp}_{l.o}= (3494.8\pm 24.7)\times10^{-9} $ which leads to : $\Delta a_\mu\equiv a_\mu^{exp}-a_\mu^{th} = (143\pm 42_{th}\pm 22_{exp})\times 10^{-11}$ indicating about 3$\sigma$ discrepancy between the SM predictions and experiment. One also finds: $\alpha^{(5)}(M_Z)\vert_{had}=(2766.3\pm 4.5)\times 10^{-5}$.

==> bib_e+e-summary.tex <==
 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{thebibliography}{999}
\vspace*{-0.15cm}
 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\bibitem{SNe} S. Narison, arXiv: 2306.14639 [hep-ph] (to appear in  {\it Nucl. Phys.} {\bf A}  (2023).
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% EXPERIMENT
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\bibitem{PDG}R.L. Workman et al. (Particle Data Group), {\it Prog. Theor. Exp. Phys.}  {\bf 2022} (2022) 083C01.

\bibitem{CMD3}CMD-3 Collaboration - F.V. Ignatov et al., 2302.08834 [hep-ex] (2023).

%%%%%%%%%%%%%%%%%%%
% QSSR SVZ & REVIEW
%%%%%%%%%%%%%%%%%%%
\bibitem{SVZa}M.A. Shifman, A.I. Vainshtein, V.I. Zakharov, {\it Nucl. Phys.} {\bf B147} (1979) 385; {\it ibid}, 
%\bibitem{SVZb}M.A. Shifman, A.I. Vainshtein and V.I. Zakharov, 
{\it Nucl. Phys.} {\bf B147} (1979) 448.

%%%%%%%%%%%%%%%%%%%
% QSSR SVZ & REVIEW
%%%%%%%%%%%%%%%%%%%
\bibitem{ZAKA}V.I. Zakharov, 
%talk given at the Sakurai's Price, 
{\it Int. J. Mod .Phys.} {\bf  A14}, (1999) 4865.
 \bibitem{SNB1} S. Narison, {\it QCD spectral sum rules, World Sci. Lect. Notes Phys.} {\bf 26} (1989) 1.
\bibitem{SNB2}S. Narison, {\it QCD as a theory of hadrons, Cambridge Monogr. Part. Phys. Nucl. Phys. Cosmol.} {\bf 17}.
 (2004) 1-778 [hep-ph/0205006]. 
 \bibitem{SNREV1}S. Narison, {\it Nucl. Part. Phys. Proc.}{\bf  312-317} (2021) 87;  
 %{\it Nucl. Part. Phys. Proc.} 
 ibid, {\bf 258-259} (2015) 189. 

%%%%%%%%%%%%%%%%%%%
% LAPLACE SUM RULE
%%%%%%%%%%%%%%%%%%%
\bibitem{SNR}S. Narison and E. de Rafael,  {\it Phys. Lett.} {\bf B 103},  (1981) 57.
\bibitem{BELLa}J.S. Bell and R.A. Bertlmann, {\it Nucl. Phys.} {\bf B177}, (1981) 218; 
%\bibitem{BELLb}J.S. Bell and R.A. Bertlmann, 
{\it Nucl. Phys.} {\bf B187}, (1981) 285.
%%%%%%%%%%%%%%%%%%%%%%
% RENORMALIZATION OF OPERATORS
%%%%%%%%%%%%%%%%%%%%%%%
\bibitem{SNTARRACH}S. Narison, R. Tarrach, {\it Phys. Lett.} {\bf B125} (1983) 217;
M. Jamin, M. Kremmer, {\it Nucl. Phys.} 
{\bf B277} (1986)  349.

    %%%%%%%%%%%%%%%%%%%%
  % QCD PARAMETERS CORRELATIONS
  %%%%%%%%%%%%%%%%%%%%
  \bibitem{SNparam}S. Narison,  {\it Int. J. Mod. Phys.} {\bf A33} (2018) no. 10, 185004; %\, [	arXiv:1801.00592 [hep-ph]].
%  \bibitem{SNparama} S. Narison, 
  Addendum: {\it Int. J. Mod. Phys.} {\bf A33} (2018) no.10, 1850045.% [arXiv:1812.09360 [hep-ph]].
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\bibitem{SNcb1}S. Narison,  {\it Phys. Lett.} {\bf B693}  (2010) 559, erratum {\it ibid}, %{\it Phys. Lett.} 
{\bf B705} (2011) 544; 
%\bibitem{SNcb2}S. Narison,  
%{\it Phys. Lett.}
ibid, {\bf B706}  (2012) 412; 
%\bibitem{SNcb3}S. Narison,  
%{\it Phys. Lett.}
ibid, {\bf B707}  (2012) 259.

%%%%%%%%%%%%%%%%%%%
% REVIEW OF  LAPLACE SUM RULE
%%%%%%%%%%%%%%%%%%%
\bibitem{SNLSR} For a recent review, see e.g. S. Narison, invited contribution to the book {\it The Laplace Transform and its Applications}, edited by Nova Science Publishers, New-York - 2023 (arXiv: 2309.00258 [hep-ph]).

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 %  RATIO OF MOMENTS
 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\bibitem{LNT}G. Launer, S. Narison, R. Tarrach, {\it  Z. Phys.} {\bf C26}
(1984) 433.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 %  FESR
 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\bibitem{FESR}R.A. Bertlmann, G. Launer and E. de Rafael, {\it Nucl. Phys.} {\bf B250}, (1985) 61;  R.A. Bertlmann, C.A. Dominguez, M. Loewe, M. Perrottet and E. de Rafael, {\it Z. Phys.} {\bf C39} (1988) 231.


\bibitem{BOITO}  D. Boito, S. Carlos. M. Golterman, K. Maltman, S. Peris, M.V. Rodrigues, arXiv\,: 2112.05413 [hep-ph] (20121) and references quoted therein.

\bibitem{PICH1} A. Pich, A. Rodriguez-Sanchez, {\it Phys.Rev.} {\bf D94} (2016) 3, 034027.

\bibitem{SN95}S. Narison, {\it Phys. Lett.}  {\bf B361} (1995) 121;


%\bibitem{DAVIER} M. Davier, A. H\"ocker, B. Malaescu, C. Z. Yuan, Z. Zhang, {\it Eur. Phys. J.} {\bf C74} (2014) 2803.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% D=2
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\bibitem{CNZa} K.G. Chetyrkin, S. Narison and V.I. Zakharov, {\it Nucl. Phys.} 
{\bf B550} (1999)  353.

\bibitem{KAHN} M.S.A. Alam Khan, arXiv: 2306.10262 (2023).

\bibitem{SNPICH} S. Narison,  A. Pich, {\it Phys. Lett.} {\bf B304} (1993) 359.
 
 \bibitem{BNP}E. Braaten, S. Narison, A. Pich, {\it Nucl. Phys.} {\bf B373} (1992) 581.
 
 \bibitem{ALEPH} The ALEPH Collaboration-R. Barate et al., {\it Eur. Phys. J.} {\bf C4} (1998) 409.

\bibitem{OPAL} The OPAL Collaboration-K. Ackerstaff et al., {\it Eur. Phys. J.} {\bf C7} (1999) 571.

\bibitem{SNTAU}S. Narison, {\it Phys. Lett.} {\bf B673} (2009) 30.

\bibitem{CHET4}P. A. Baikov, K.G. Chetyrkin.J.H. K\"uhn, {\it Phys.Rev.Lett.} {\bf 101}(2008) 012002. 

\bibitem{DAVIER} M. Davier, A. H\"ocker, B. Malaescu, C. Z. Yuan, Z. Zhang, {\it Eur. Phys. J.} {\bf C74} (2014) 2803.

\bibitem{PICH2} A. Pich, A. Rodriguez-Sanchez,{\it Mod.Phys.Lett.} {\bf A31} (2016) 30, 1630032; {\it Journal of High Energy Physics} {\bf  145} (2022).



%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 % AMU
 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  \bibitem{CALMET} J. Calmet, S. Narison, M. Perrottet and E. de Rafael, {\it Phys. Lett.} {\bf B161} (1976) 283; {\it Rev. Mod. Phys.} {\bf 49} (1977)21.
 \bibitem{SN76} S. Narison, {\it Th\`ese de 3 \`eme cycle}, Univ. Marseille Luminy (1976) unpublished.
   \bibitem{SNamu}S. Narison, {\it Phys. Lett.} {\bf B513} (2001) 53;  {\bf Phys. Lett.} {\bf B526} (2002) 414 (erratum).
     \bibitem{SN78} S. Narison, {\it J. Phys.: Nucl. Phys.} {\bf G4} (1978) 1849.  
     \bibitem{SNalfa}S. Narison, arXiv: 0108065[hep-ph] (2001). 

     
\bibitem{BOUCHIAT} C. Bouchiat and L. Michel, {\it J. Phys. Radium} {\bf 22}
(1961) 121.
\bibitem{DURAND} L. Durand III, {\it Phys. Rev.} {\bf 128} (1962) 441; erratum {\bf 129} (1963) 2835.
\bibitem{KINOSHITA}T. Kinoshita and R. Oakes, {\it Phys. Lett.} {\bf B25}(1967) 143.
\bibitem{BOWCOCK}J.E. Bowcock, {\it Z. Phys.} {\bf 211} (1968) 400.
\bibitem{GOURDIN}M. Gourdin and E. de Rafael, {\it Nucl. Phys.} {\bf B10} (1969) 667.
\bibitem{LAUTRUP}B. Lautrup and E. de Rafael, {\it Phys. Rev.} {\bf 174} (1968) 1835.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 % AMU FIT
 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\bibitem{NOMURA}A. Keshavarzi, D. Nomura, T. Teubner, {\it Phys. Rev.} {\bf D101} (2020) 014029.
\bibitem{DAVIER2} M. Davier, A. H\"ocker, B. Malaescu,  Z. Zhang, {\it Eur. Phys. J.} {\bf C80} (2020) 241.
 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 \bibitem{MIRANDA} P. Masjuan, A. Miranda, P. Roig, arXiv:2305.20005 (2023) and private communication from A. Miranda. 
 \bibitem{RAF} E. de Rafael, {\it Phys. Lett.} {\bf B736} (2014) 522.
 \bibitem{GM2}T. Aoyama et al., {\it  Phys. Rept.} {\bf 887} (2020)1 and references therein.
 \bibitem{LATTICE}Sz. Borsanyi et al. {\it  Nature} {\bf 593(7857)} (2021)51;  Marco C`e et al.,
{\it  Phys. Rev.} {\bf D106(11)} (2022)114502; C. Alexandrou et al., {\it PoS ICHEP 2022} (2022) 794; T. Blum et al., arXiv:  2301.08696 [hep-lat] (2023).
 \bibitem{KNECHT} M. Knecht, S. Narison, A. Rabemananjara, D. Rabetiarivony
 {\it Phys. Lett.} {\bf B787} (2018) 111.
 \bibitem{BNL} G. Bennett et al., {\it Phys. Rev.} {\bf D73} (2006) 072003.
\bibitem{FNAL}    B. Abi et al., {\it Phys. Rev. Lett.} {\bf 126} (2021) 141801;  T. Albahri et al., {\it Phys. Rev.} {\bf  D103} (2021) 072002.

\bibitem{YND17}J. F. de Troconiz, F. J. Yndurain, {\it Phys. Rev.} {\bf D65} (2002) 093002.
\bibitem{JEGER} F. Jegerlehner, {\it CERN Yellow Reports: Monographs} {\bf 3} (2020) 9.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\end{thebibliography}
\end{document}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

  
  
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%  AMU-ALFA 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 \bibitem{CALMET} J. Calmet, S. Narison, M. Perrottet and E. de Rafael, {\it Phys. Lett.} {\bf B161} (1976) 283; {\it Rev. Mod. Phys.} {\bf 49} (1977)21.
 \bibitem{SN76} S. Narison, {\it Th\`ese de 3 \`eme cycle}, Univ. Marseille Luminy (1976) unpublished. 
  \bibitem{SNamu}S. Narison, {\it Phys. Lett.} {\bf B513} (2001) 53;  {\bf Phys. Lett.} {\bf B526} (2002) 414 (erratum).
  \bibitem{SN78} S. Narison, {\it J. Phys.: Nucl. Phys.} {\bf G4} (1978) 1849.  
\bibitem{SNalfa}S. Narison, arXiv: 0108065[hep-ph] (2001). 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%% RENORMALIZATION OF OCNDENSATES%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\bibitem{ESPRIU}
 \bibitem{TARRACH}R. Tarrach, {\it Nucl.Phys.} {\bf B 196} (1982) 45.
\bibitem{ESPRIU}D. Espriu and R. Tarrach, {\it Z. Phys.} {\bf C 16}, (1982) 77.
\bibitem{SNTARRACH}S. Narison, R. Tarrach, {\it Phys. Lett.} {\bf B125} (1983) 217;
M. Jamin, M. Kremmer, {\it Nucl. Phys.} 
{\bf B277} (1986)  349.

\bibitem{BAGAN} E. Bagan, J.I. Latorre, P. Pascual, R. Tarrach, {\it Nucl. Phys.} 
{\bf B254} (1985)  555.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% ORDER ALPHAS 3, 4
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\bibitem{LARIN} S.G. Gorishny, A.L. Kataev, S.A. Larin, {\it  Phys. Lett.}  {\bf B259} (1991)  144; L.R. Surguladze, M.A. Samuel, {\it  Phys. Rev. Lett.} 
{\bf 66} (1991)  560.

\bibitem{CHET4}P. A. Baikov, K.G. Chetyrkin.J.H. K\"uhn, {\it Phys.Rev.Lett.} {\bf 101}(2008) 012002. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% D=2
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\bibitem{CNZa} K.G. Chetyrkin, S. Narison and V.I. Zakharov, {\it Nucl. Phys.} 
{\bf B550} (1999)  353.
\bibitem{SZ}S. Narison and V.I. Zakharov, {\it Phys. Lett.} {\bf B679} (2009) 355.
\bibitem{CNZb}S. Narison and V.I. Zakharov, {\it  Phys. Lett.} {\bf B522} (2001) 266.
\bibitem{D2rev} For reviews, see e.g.: V.I. Zakharov, {\it Nucl. Phys. Proc. Suppl.} 
{\bf 164} (2007) 240; S. Narison,  {\it Nucl. Phys. Proc. Suppl.} {\bf 164} (2007) 225.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\bibitem{ADS1}	O. Andreev, {\it Phys. Rev.} {\bf D73} (2006) 107901; 
%\bibitem{ADS2}	
O. Andreev, V.I. Zakharov,  {\it Phys. Rev.} {\bf D74} (2006) 025023; {\it ibid}, {\bf D76} (2007)047705.
\bibitem{ADS3}	 F. Jugeau, S. Narison, H. Ratsimbarison,  {\it Phys. Lett.}  {\bf  B722} (2013) 111.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% D=2 FIT 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\bibitem{SN93}S. Narison, {\it Phys. Lett.}  {\bf B300} (1993) 293
\bibitem{SN95}S. Narison, {\it Phys. Lett.}  {\bf B361} (1995) 121;
\bibitem{SNTAU}S. Narison, {\it Phys. Lett.} {\bf B673} (2009) 30.
\bibitem{TERAYEV} M. Kozhevnikova, A. Oganesian and O. Terayev, EPJ Web of Conferences 204 (2019) 02005.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% D=4 FIT 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 % D=8
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\bibitem{MALLIK} W. Hubschmid, S. Mallik, {\it Nucl. Phys.} {\bf B207}, (1982) 29;
M.S. Dubovikov, A.V. Smilga, {\it Nucl. Phys.} {\bf B185}, (1981) 109.
\bibitem{BROAD8} D. Broadhurst, S. Generalis, {\it  Phys. Lett.} 
{\bf B165} (1985)  175.

   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 %  D=8
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% EXPERIMENT
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\bibitem{PDG}R.L. Workman et al. (Particle Data Group), {\it Prog. Theor. Exp. Phys.}  {\bf 2022} (2022) 083C01.

\bibitem{CMD3}CMD-3 Collaboration - F.V. Ignatov et al., 2302.08834 [hep-ex] (2023).

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\bibitem{KAHN2} M.S.A Alam Kahn (private communication).
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%  TAU-DECAY
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\bibitem{BOITO}  D. Boito, S. Carlos. M. Golterman, K. Maltman, S. Peris, M.V. Rodrigues, arXiv\,: 2112.05413 [hep-ph] (20121) and references quoted therein.

\bibitem{ALEPH} The ALEPH Collaboration-R. Barate et al., {\it Eur. Phys. J.} {\bf C4} (1998) 409.

\bibitem{OPAL} The OPAL Collaboration-K. Ackerstaff et al., {\it Eur. Phys. J.} {\bf C7} (1999) 571.

\bibitem{PICH1} A. Pich, A. Rodriguez-Sanchez, {\it Phys.Rev.} {\bf D94} (2016) 3, 034027.


\bibitem{DAVIER} M. Davier, A. H\"ocker, B. Malaescu, C. Z. Yuan, Z. Zhang, {\it Eur. Phys. J.} {\bf C74} (2014) 2803.

\bibitem{PICH2} A. Pich, A. Rodriguez-Sanchez,{\it Mod.Phys.Lett.} {\bf A31} (2016) 30, 1630032; {\it Journal of High Energy Physics} {\bf  145} (2022).

 \bibitem{LEDI}F. Le Diberder,  A. Pich, {\it Phys. Lett.} {\bf B286} (1992) 147; {\bf B289} 
(1992) 165.

\bibitem{BNP2}E. Braaten, {\it Phys. Rev. Lett.} {\bf 60} (1988) 606; E. Braaten, {\it Phys. Rev.} {\bf D39} (1989) 1458; S. Narison, A. Pich, {\it Phys. Lett.} {\bf B211} (1988) 183.

\bibitem{BNP}E. Braaten, S. Narison, A. Pich, {\it Nucl. Phys.} {\bf B373} (1992) 581.



%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 %  RATIO OF CONDENSATES
 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\bibitem{SOLA} C.A. Dominguez, J. Sola, {\it  Z. Phys.} {\bf C40} (1988) 63.

\bibitem{BORDES} J. Bordes, V. Gimenenz, J.A. Penarrocha, {\it Phys. Lett.} {\bf B201} (1988) 365.

\bibitem{CAUSSE} M.B. Causse, G. Mennessier, {\it  Z. Phys.} {\bf C47} (1990) 611.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 %  LAPLACE - TAU-LIKE
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\bibitem{EIDELMAN} S.I. Eidelman, L.M. Kurdadze, A.I. Vainshtein,  {\it Phys. Lett.} {\bf B82} (1979) 278.

\bibitem{KAHN} M.S.A. Alam Khan, arXiv: 2306.10262 (2023).

 \bibitem{SNPICH} S. Narison,  A. Pich, {\it Phys. Lett.} {\bf B304} (1993) 359.
 
 \bibitem{JAMIN} M. A. Benitez-Rathgeb, D. Boito,  A.H. Hoang, M. Jamin, {\it JHEP} {\bf 09} (2022) 223;
 {\it ibid} {\bf 07} (2022) 016.
 
  \bibitem{RENORM}M. Beneke, M. Jamin, {\it JHEP} {\bf 044} (2008) 0809.
  
 \bibitem{AYALA} C. Ayala, G. Cvetic, D. Teca, {\it Eur. Phys. J.} {\bf C81}  (2021) 930.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 % AMU
 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\bibitem{BOUCHIAT} C. Bouchiat and L. Michel, {\it J. Phys. Radium} {\bf 22}
(1961) 121.
\bibitem{DURAND} L. Durand III, {\it Phys. Rev.} {\bf 128} (1962) 441; erratum {\bf 129} (1963) 2835.
\bibitem{KINOSHITA}T. Kinoshita and R. Oakes, {\it Phys. Lett.} {\bf B25}(1967) 143.
\bibitem{BOWCOCK}J.E. Bowcock, {\it Z. Phys.} {\bf 211} (1968) 400.
\bibitem{GOURDIN}M. Gourdin and E. de Rafael, {\it Nucl. Phys.} {\bf B10} (1969) 667.
\bibitem{LAUTRUP}B. Lautrup and E. de Rafael, {\it Phys. Rev.} {\bf 174} (1968) 1835.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\bibitem{CHETmass} K.G. Chetyrkin, J.H. K\"uhn,A. Kwiatkowski, {\it Phys. Lett.} {\bf B282} (1992) 221; K.G. Chetyrkin, J.H. K\"uhn, {\it Nucl. Phys.} {\bf B432} (1994) 337.
\bibitem{FNR}E.G. Floratos, S. Narison, E. de Rafael, {\it Nucl. Phys.} {\bf B155} (1979) 115.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 % AMU FIT
 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\bibitem{NOMURA}A. Keshavarzi, D. Nomura, T. Teubner, {\it Phys. Rev.} {\bf D101} (2020) 014029.
\bibitem{DAVIER2} M. Davier, A. H\"ocker, B. Malaescu,  Z. Zhang, {\it Eur. Phys. J.} {\bf C80} (2020) 241.
 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 \bibitem{MIRANDA} P. Masjuan, A. Miranda, P. Roig, arXiv:2305.20005 (2023) and private communication from A. Miranda. 
 \bibitem{RAF} E. de Rafael, {\it Phys. Lett.} {\bf B736} (2014) 522.
 \bibitem{GM2}T. Aoyama et al., {\it  Phys. Rept.} {\bf 887} (2020)1 and references therein.
 \bibitem{LATTICE}Sz. Borsanyi et al. {\it  Nature} {\bf 593(7857)} (2021)51;  Marco C`e et al.,
{\it  Phys. Rev.} {\bf D106(11)} (2022)114502; C. Alexandrou et al., {\it PoS ICHEP 2022} (2022) 794; T. Blum et al., arXiv:  2301.08696 [hep-lat] (2023).
 \bibitem{KNECHT} M. Knecht, S. Narison, A. Rabemananjara, D. Rabetiarivony
 {\it Phys. Lett.} {\bf B787} (2018) 111.
 \bibitem{BNL} G. Bennett et al., {\it Phys. Rev.} {\bf D73} (2006) 072003.
\bibitem{FNAL}    B. Abi et al., {\it Phys. Rev. Lett.} {\bf 126} (2021) 141801;  T. Albahri et al., {\it Phys. Rev.} {\bf  D103} (2021) 072002.
\bibitem{YND17}J. F. de Troconiz, F. J. Yndurain, {\it Phys. Rev.} {\bf D65} (2002) 093002.
\bibitem{JEGER} F. Jegerlehner, {\it CERN Yellow Reports: Monographs} {\bf 3} (2020) 9.
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\end{thebibliography}
\end{document}
 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%



